Synthetic Data for Model Selection

Recent breakthroughs in synthetic data generation approaches made it possible to produce highly photorealistic images which are hardly distinguishable from real ones. Furthermore, synthetic generation pipelines have the potential to generate an unlimited number of images. The combination of high photorealism and scale turn synthetic data into a promising candidate for improving various machine learning (ML) pipelines. Thus far, a large body of research in this field has focused on using synthetic images for training, by augmenting and enlarging training data. In contrast to using synthetic data for training, in this work we explore whether synthetic data can be beneficial for model selection. Considering the task of image classification, we demonstrate that when data is scarce, synthetic data can be used to replace the held out validation set, thus allowing to train on a larger dataset. We also introduce a novel method to calibrate the synthetic error estimation to fit that of the real domain. We show that such calibration significantly improves the usefulness of synthetic data for model selection.

==> customer_impact.tex <==
\section*{Customer Impact}
Deploying the best possible model for Amazon customers' benefit is very important. That said, in today's common practice, model selection depends largely on the evaluation set being used for assessing the model's generalization capabilities. Such sequestered dataset usually comes at the price of reducing the training dataset size. In this work we propose to leverage the power of Generative Adversarial Networks (GANs) for creating such evaluation dataset to eliminate the need for holding out portions of real data. This real data can be instead used for training, to improve the performance of the deployed models.



==> figures/fig_architecture_search.tex <==
\newcommand{\centered}[1]{\begin{tabular}{@{}l@{}} #1 \end{tabular}}
\begin{figure}
\centering
\begin{tabular}{c c c}
Train50K & Train30K & Train10K \\
\includegraphics[width=0.3\linewidth]{images/arc_search/50K_points.png} &
\includegraphics[width=0.3\linewidth]{images/arc_search/30K_points.png} &
\includegraphics[width=0.3\linewidth]{images/arc_search/10K_points.png} \\
\includegraphics[width=0.3\linewidth]{images/arc_search/50K_10_best.png} &
\includegraphics[width=0.3\linewidth]{images/arc_search/30K_10_best.png} &
\includegraphics[width=0.3\linewidth]{images/arc_search/10K_10_best.png}

\end{tabular}

% \renewcommand{\arraystretch}{2}
% \begin{tabular}{c c c}
%     \centered{a} &
% \includegraphics[width=0.4\linewidth]{images/arc_search/50K_points.png} & 
% \includegraphics[width=0.4\linewidth]{images/arc_search/50K_10_best.png} \\
% \rotatebox{90}{Train50K} &
% \includegraphics[width=0.4\linewidth]{images/arc_search/50K_points.png} & 
% \includegraphics[width=0.4\linewidth]{images/arc_search/50K_10_best.png} \\
% \rotatebox{90}{Train50K} &
% \includegraphics[width=0.4\linewidth]{images/arc_search/50K_points.png} & 
% \includegraphics[width=0.4\linewidth]{images/arc_search/50K_10_best.png} \\

% \end{tabular}

\caption{\textbf{Synthetic data for architecture hyper-parameters search:} graphs are place holders}

\label{fig:architecture_search}
\end{figure}

==> figures/fig_big_gan_107.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{ c  c}
%    \hline
    Jellyfish (precision: $1$, recall: $0$)  & Spindle (precision: $0.15$, recall: $0.74$) \\
    %\hline
    \includegraphics[width=0.4\linewidth]{images/biggan/grid_107.png} &
    \includegraphics[width=0.4\linewidth]{images/biggan/grid_816.png}
  \end{tabular}
 
% \captionsetup{belowskip=0pt}
% \setlength{\belowcaptionskip}{100pt}
\setlength{\floatsep}{500pt}
% \setlength{\textfloatsep}{200pt}
\caption{\textbf{BigGAN samples}: (left) The class with the highest precision. 
(right) The class with the highest recall.}
\label{fig:biggan_samples}
\end{figure}




==> figures/fig_biggan.tex <==
\begin{figure}
%   \centering
%   \includegraphics[width=0.5\linewidth]{images/es_rs/barplots_all.png}
\centering

\begin{tabular}{c c}
    \includegraphics[height=0.35\linewidth]{images/biggan/correlation_top1.pdf} &
    \includegraphics[height=0.35\linewidth]{images/biggan/precision_recall_imagenet.pdf}
\end{tabular}    

\caption{\textbf{Results for BigGAN:} (Left) Each point represents the test error (x axis), $\hat{\epsilon_r}$, and synthetic data error (y axis), $\hat{\epsilon_s}$, of a single model.
(Right) Precision and recall for each class. 
The color of each point represents the Spearman's correlation coefficient between the error of classifiers per class.
Points with a black cross represent classes where all classifiers have identical error.
There are 548 such points out of the 1000 classes.
}
\label{fig:biggan}
\end{figure}



==> figures/fig_imagenet_intresting.tex <==
\begin{figure}
    \centering
    \setlength{\tabcolsep}{2pt}
    %\renewcommand{\arraystretch}{0.5} % Default value: 1
    \begin{tabular}{ c c c}
%    \hline
     $w=0.0$ & $w=0.064$ &  \\
     \rotatebox{90}{\hspace{4mm}\tiny{Class 250, DiT (cfg=1) \textcolor{white}{p}}}
     \includegraphics[width=0.31\linewidth]{images/imagenet_intresting/250_0000001.png} &
     \includegraphics[width=0.31\linewidth]{images/imagenet_intresting/250_0000030.png} &
     \includegraphics[width=0.31\linewidth]{images/imagenet_intresting/image (21).png} \\
     $w=0.041$ & $w=-0.012$ &  \\
     \rotatebox{90}{\hspace{4mm}\tiny{Class 608, DiT (cfg=4) \textcolor{white}{p}}}
     \includegraphics[width=0.31\linewidth]{images/imagenet_intresting/608_0000061.png} &
     \includegraphics[width=0.31\linewidth]{images/imagenet_intresting/608_0000067.png} &
     \includegraphics[width=0.31\linewidth]{images/imagenet_intresting/image (22).png} \\
     
     



    \end{tabular}
 
\caption{\textbf{TODO:} .}
\label{fig:fig_imagenet_intresting}
\end{figure}




==> figures/fig_imagenet_intresting_sampels.tex <==
\begin{figure}[H]
\begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=0.99\linewidth]{images/imagenet_w/cfg_4_250/4.jpg}
    %\vskip -0.1in
    \caption{DiT (cfg $=4$)}
    \label{fig:a}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=0.99\linewidth]{images/imagenet_intresting/250_0000001.png}
    %\vskip -0.1in
    \caption{BigGAN}
    \label{fig:a}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=0.99\linewidth]{images/imagenet_intresting/608_0000061.png}
    %\vskip -0.1in
    \caption{BigGAN}
    \label{fig:a}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=0.99\linewidth]{images/imagenet_intresting/608_0000067.png}
    %\vskip -0.1in
    \caption{BigGAN}
    \label{fig:a}
\end{subfigure}
 
\caption{\textbf{Calibrated samples of class ``Siberian husky'' (250):}
First row, columns 3 shown an image that received a low negative number.
It appears that this is a failure of the generative model, as it produced that is more similar to class 248 (Eskimo dog, husky) rather than to the intended class (Siberian Husky). 
Of the models in the calibration set, 21 models classified it as 248 while 29 models classified it as 250, where the highest performing models predicted 248.
Therefore this image is useful for ranking since high performing models tend to agree that this is not a Siberian husky.
First and second row, column 5, received the weight of 0.
The first row received 0 since all classifiers were able to predict the class correctly.
While the image in the second row was ...
First column, second row -- }

% Each row shows images from a different synthetic dataset.
% The first four columns show the images that received the highest positive and lowest negative $w$ coefficient values during calibration.
% Columns five and six show samples that are not useful for ranking and received $w=0$.
% These images are either labeled correctly by all calibration models or labeled ``incorrectly'' by all of them. 
% The last column shows the distribution of $w$ for all 100 images in the class.}
\label{fig:fig_imagenet_w_intresting}
\end{figure}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/table_early_stopping_random_seed.tex <==
\begin{table}[b]
  \setlength{\textwidth}{0pt}
  \centering
  \small
  \begin{tabular}{c}
    \underline{Train50K}
  \end{tabular}
  
  \begin{tabular}{ c | c | c | c | c | c | c || c}
      & example net & Vgg & resNet18 & denseNet & TBD & TBD & Avg delta\\ \hline
    Last epoch & $97.8$\tiny{$\pm0.5$} & TBD & TBD & TBD & TBD & TBD & TBD\\ \hline
    ES &         $98.8$\tiny{$\pm0.2$} & TBD & TBD & TBD & TBD & TBD & TBD\\ \hline
    RS &         $98.1$ & TBD & TBD & TBD & TBD & TBD & TBD\\ \hline
    ES + RS &    $98.2$ & TBD & TBD & TBD & TBD & TBD & TBD
  \end{tabular}
    \caption{\textbf{}}
    \label{tab:early_stopping_random_seed}
\end{table}

==> tables/table_of_archs.tex <==
\begin{table}
\begin{center}
    \begin{tabular}{ c | c | c | c }
%    \hline
    \multicolumn{4}{c}{Train50K} \\
    \hline
    Architecture & Orig-Error & Synth-Class-Error & Synth-Cond-Error \\
    \hline
    vgg & TBD & TBD & TBD \\ \hline
    densenet & TBD & TBD & TBD\\ \hline
    resnet & TBD & TBD & TBD\\ \hline
  \end{tabular}
\end{center}
    \caption{\textbf{TBD}}
    \label{tab:table_of_models_errors_tr50}
\end{table}



==> tables/table_one_arch_10_runs.tex <==
\begin{table}
\begin{center}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrr}
\hline
    architecture\_name &  train\_size &  train\_\# &  best\_test\_acc &  best\_vs\_epoch &  best\_vs\_acc &  test\_at\_best\_vs &  best\_vcs\_epoch &  best\_vcs\_acc &  test\_at\_best\_vcs &  best\_wgan\_class\_epoch &  best\_wgan\_class\_acc &  test\_at\_best\_wgan\_class &  best\_wgan\_cond\_epoch &  best\_wgan\_cond\_acc &  test\_at\_best\_wgan\_cond &  test\_acc\_at\_last\_epoch &  vs\_acc\_at\_last\_epoch &  vcs\_acc\_at\_last\_epoch &  wgan\_class\_acc\_at\_last\_epoch &  wgan\_cond\_acc\_at\_last\_epoch \\
\hline
 resnet\_tr50\_basic\_32 &        4096 &        0 &          76.04 &            159 &       77.858 &            75.95 &             156 &        72.015 &             75.98 &                    159 &               77.557 &                    75.95 &                   159 &              69.593 &                   75.95 &                   75.95 &                77.858 &                 71.987 &                        77.557 &                       69.593 \\
 resnet\_tr50\_basic\_32 &        4096 &        1 &          84.70 &            150 &       85.894 &            84.59 &              96 &        78.632 &             84.48 &                    159 &               79.222 &                    84.48 &                   159 &              70.193 &                   84.48 &                   84.48 &                85.876 &                 78.571 &                        79.222 &                       70.193 \\
 resnet\_tr50\_basic\_32 &        4096 &        2 &          78.77 &            155 &       80.297 &            78.71 &             154 &        74.204 &             78.77 &                    159 &               77.807 &                    78.73 &                   159 &              70.478 &                   78.73 &                   78.73 &                80.280 &                 74.145 &                        77.807 &                       70.478 \\
 resnet\_tr50\_basic\_32 &        4096 &        3 &          77.86 &            153 &       79.387 &            77.73 &             153 &        73.261 &             77.73 &                    159 &               77.385 &                    77.69 &                   159 &              69.661 &                   77.69 &                   77.69 &                79.339 &                 73.258 &                        77.385 &                       69.661 \\
 resnet\_tr50\_basic\_32 &        4096 &        4 &          83.62 &            149 &       84.437 &            83.52 &             149 &        77.837 &             83.52 &                    159 &               80.814 &                    83.44 &                   159 &              71.975 &                   83.44 &                   83.44 &                84.326 &                 77.796 &                        80.814 &                       71.975 \\
 resnet\_tr50\_basic\_32 &        4096 &        5 &          81.89 &            159 &       82.893 &            81.81 &             130 &        76.795 &             81.76 &                    159 &               79.352 &                    81.81 &                   159 &              71.096 &                   81.81 &                   81.81 &                82.893 &                 76.753 &                        79.352 &                       71.096 \\
 resnet\_tr50\_basic\_32 &        4096 &        6 &          84.26 &            146 &       85.517 &            84.22 &             122 &        78.338 &             83.99 &                    159 &               77.701 &                    84.10 &                   159 &              69.198 &                   84.10 &                   84.10 &                85.489 &                 78.257 &                        77.701 &                       69.198 \\
 resnet\_tr50\_basic\_32 &        4096 &        7 &          83.76 &            155 &       84.945 &            83.70 &             158 &        77.962 &             83.61 &                    159 &               81.356 &                    83.63 &                   159 &              72.023 &                   83.63 &                   83.63 &                84.892 &                 77.953 &                        81.356 &                       72.023 \\
 resnet\_tr50\_basic\_32 &        4096 &        8 &          84.00 &            146 &       85.525 &            83.98 &             155 &        78.623 &             83.93 &                    159 &               80.785 &                    83.97 &                   159 &              71.929 &                   83.97 &                   83.97 &                85.477 &                 78.593 &                        80.785 &                       71.929 \\
 resnet\_tr50\_basic\_32 &        4096 &        9 &          82.08 &            151 &       83.694 &            81.99 &             120 &        76.685 &             81.79 &                    159 &               79.789 &                    81.90 &                   159 &              70.952 &                   81.90 &                   81.90 &                83.643 &                 76.636 &                        79.789 &                       70.952 \\
\hline
\end{tabular}
\end{center}
    \caption{\textbf{TBD}}
    \label{tab:table_one_arch_10_runs}
\end{table}


